Differentiable Discrete Elastic Rods for Real-Time Modeling of Deformable Linear Objects

This paper addresses the task of modeling Deformable Linear Objects (DLOs), such as ropes and cables, during dynamic motion over long time horizons. This task presents significant challenges due to the complex dynamics of DLOs. To address these challenges, this paper proposes differentiable Discrete Elastic Rods For deformable linear Objects with Real-time Modeling (DEFORM), a novel framework that combines a differentiable physics-based model with a learning framework to model DLOs accurately and in real-time. The performance of DEFORM is evaluated in an experimental setup involving two industrial robots and a variety of sensors. A comprehensive series of experiments demonstrate the efficacy of DEFORM in terms of accuracy, computational speed, and generalizability when compared to state-of-the-art alternatives. To further demonstrate the utility of DEFORM, this paper integrates it into a perception pipeline and illustrates its superior performance when compared to the state-of-the-art methods while tracking a DLO even in the presence of occlusions. Finally, this paper illustrates the superior performance of DEFORM when compared to state-of-the-art methods when it is applied to perform autonomous planning and control of DLOs. Project page: https://roahmlab.github.io/DEFORM/.

==> revision_text/DER.tex <==
\section{Model DLO with Discrete Elastic Rods(DER)}



\begin{figure}
    \centering
     \includegraphics[width=0.4\textwidth]{figures/DER_with_robot.png}
     \caption{\textbf{DER Setting with Robots: Need to be edited}}
    \label{fig:primal-dual}
\end{figure}

\textbf{Derivation for DER:}\\
$\textbf{e}_\text{t}^\text{i} \in \mathbb{R}^3$ which is defined as $\textbf{x}^{i+1} - \textbf{x}^{i}$. 
$\overline{\textbf{e}}$ represents the natural configuration of wire \Ram{what does that mean? Like the edges?}.
All barred quantities in the following represent the natural configuration (without external/internal force) of wires. 
Notice that the natural configuration of the wire is not necessarily straight or a parabolic shape.\\ 
\textbf{Adaptive Frame Setup}:\\
\textbf{Bishop Frame}:  \Ram{it feels as if most of this should be rewritten using a definition environment (look at the RSS paper I shared with you)}
$\Gamma^\text{i}_\text{B}: {\{\textbf{t}^\text{i}, \textbf{v}_1^\text{i}, \textbf{v}_2^\text{i}\}}$. 
Define frame transport \Ram{what does frame transport mean?} using quaternion rotation $R_{\text{q}^\text{i}}(\bm{v^\text{i}})$ \Ram{this seems to be missing an equal sign of some kind? or are you saying that its defined in the equation below?}, $\text{q}^\text{i}=(\text{q}_0^\text{i}, \textbf{q}^\text{i}$), $\text{q}_0^\text{i}$ represents magnitude and $\textbf{q}^\text{i}$ represents axial vector.  

To minimize twist along the frame transport, it follows: $\textbf{q}^\text{i} \cdot \textbf{t}^\text{i} = 0$ \Ram{this is probably missing a citation}.
The equation prohibits $\Gamma_\text{B}^\text{i}$ to rotate around vector $\textbf{t}^\text{i}$, which is why it is twist-free \cite{originalDER, kirchoff}. 
Combining the equation \Ram{which equation?} with \eqref{eq:parallel transfort1_1}'s first equation, $\text{q}_\text{i}$ can be determined as following:
% \begin{align}
% \text{q}_0^\text{i} &= \text{cos}(\phi^\text{i}/2) 
% \label{eq:parallel transfort2_1}\\
% \textbf{q}^\text{i} &= \text{sin}(\phi^\text{i}/2)|\textbf{t}^\text{i} \times \textbf{t}^{\text{i}+1}|. 
% \label{eq:parallel transfort2_2}
% \end{align}
$\phi_\text{i}$ from Fig.\ref{fig:adapted-frame} can be determined from the magnitude of discrete curvature binormal $(\kappa\textbf{b})^\text{i}$, which represents changing rate of the tangent vector along the rod's length in the discrete case \Ram{what does in the discrete case mean?}.
% \begin{equation}
% 2\text{tan}(\frac{\phi^\text{i}}{2}) = |\kappa\textbf{b}^\text{i}| = |\frac{2\textbf{e}^{i-1} \times \textbf{e}^\text{i}}{|\overline{\textbf{e}}^{i-1}||\overline{\textbf{e}}^{i}| + \textbf{e}^{i-1}\cdot \textbf{e}^\text{i}}|
% \label{eq:parallel transfort2}
% \end{equation}
\textbf{Material Frame}: $\Gamma^\text{i}_\text{M}:{\{\boldsymbol{\textbf{t}}^\text{i}, \textbf{m}_1^\text{i}, \textbf{m}^2_\text{i}}\}$.\\
$\theta^\text{i}$ denotes the scalar that measures the rotation about the tangent of the  $\Gamma_\text{i}^\text{M}$ relative to the Bishop coordinate $\Gamma^\text{i}_\text{B}$ located at $\textbf{e}^\text{i}$. 
\begin{equation}
    \textbf{m}_1^\text{i}=\text{cos}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{sin}\theta^\text{i}\cdot \textbf{v}_2^\text{i}, \textbf{m}_2^\text{i}=-\text{sin}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{cos}\theta^\text{i}\cdot \textbf{v}_2^\text{i}
\end{equation}
\textbf{Natural Material Frame}:$\overline{\Gamma}_\text{M}:{\{\boldsymbol{\textbf{t}}, \overline{\textbf{m}}_1, \overline{\textbf{m}}_2}$ Special case while $\theta=0$ such that $\textbf{e} = \overline{\textbf{e}}$, $\overline{\textbf{m}}_1, \overline{\textbf{m}}_2=\overline{\textbf{u}}, \overline{\textbf{v}}$. \\
\textbf{Measurement of Elastic Energy}: \\
\textbf{stretching}: modeling stretching with energy methods will introduce unnecessary stiffness into the simulation and cause instability through integration methods. Original DER\cite{originalDER} adapts fast projection methods\cite{fast_proj} to solve following constraints \ref{inextensibility} post integration methods. 
\begin{equation}
    \textbf{e}_\text{i} \cdot \textbf{e}_\text{i} - \overline{\textbf{e}}_\text{i}\cdot\overline{\textbf{e}}_\text{i} = 0
\label{inextensibility}
\end{equation}
However, such methods require small steps to ensure convergence and stability. 
Instead, we adopt a constraint solver based on position-based dynamics\cite{PBD}.  
More details will be discussed in Section\ref{sec:inextensiblity methodology}. \\
\textbf{bending and twisting in material frame}: 
Measurement of bending $\boldsymbol{\omega}_\text{j}^\text{i}, \text{j}\in(\text{i}-1, \text{i})$ is represented by the magnitude of projection from curve's curvature $(\kappa\textbf{b})^\text{i}$ onto material frame $\textbf{m}_1^\text{i}, \textbf{m}_2^\text{i}$. Twisting is represented based on the $\theta$ difference between consecutive material frame.
\begin{equation}
    \boldsymbol{\omega}_j^\text{i} = ((\kappa\textbf{b})^\text{i}\cdot \textbf{m}_2^\text{j}, -(\kappa\textbf{b})^\text{i}\cdot \textbf{m}_1^\text{j}), \, \alpha^\text{i} = \theta^\text{i} - \theta^{i-1}
    \label{eq:bend and twist}
\end{equation}
With above equation, 
\begin{equation}
    \text{E}(\Gamma^\text{M}) = \sum^{n-1}_{i=2}\text{E}_{\text{bend}}(\Gamma_\text{M}^{i}) + \text{E}_{\text{twist}}(\Gamma_\text{M}^\text{i})
    \label{eq: total_energy}
\end{equation}
\begin{equation}
    \text{E}_{\text{bend}}(\Gamma^\text{i}_\text{M}) = \frac{1}{2\overline{l}^\text{i}}\sum^\text{i}_{\text{j}=\text{i}-1} (\boldsymbol{\omega}_j^\text{i} - \overline{\boldsymbol{\omega}}^i_\text{j})^T \cdot \overline{\text{B}}_\text{j} (\boldsymbol{\omega}^i_\text{j} - \overline{\boldsymbol{\omega}}_j^\text{i})\\
    \label{eq:bend_energy}
\end{equation}
\begin{equation}
        \text{E}_{\text{twist}}(\Gamma_\text{i}^\text{M}) = \frac{\overline{\beta}^\text{i}(\alpha^i)^2}{\overline{l}^\text{i}}
        \label{eq:twist_energy}
\end{equation}
bending modulus $\overline{\textbf{B}}_\text{i} \in \mathbb{R}^{2 \times 2}$, twsting modulus $\overline{\beta}_\text{i} \in \mathbb{R}^{2 \times 2}$. $\overline{\textit{l}}^\text{i} = |\overline{\textbf{e}}^{\text{i}-1}| + |\overline{\textbf{e}}^{\text{i}}|$. \\
\textbf{Solving $\theta$} \\
As discussed in \cite{originalDER}, energy of twisting and bending are minimized and are not subject to changes at the end of the prediction time step t+$\Delta$t. Therefore, we can formulate the following optimization problem to obtain $\theta$.
\begin{equation}
    \frac{\delta \text{E}(\Gamma^\text{M})}{\delta \theta} = 0
    \label{eq:theta_minimize}
\end{equation}

\subsection{Integration Method}
Integration is done based on the following second-order ODE.
\begin{equation}
       \textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\delta \text{E}(\Gamma^\text{M})}{\delta \textbf{X}_{t}}
       \label{eq:Integration}
\end{equation}
A detailed derivation of Eq.\ref{eq:Integration} can be found in \cite{originalDER}. DER\cite{originalDER} solves it with Semi-Euler method\cite{implicit-euler}, which has the same computational cost while having better tracking performance compared to Euler's method, as shown in the following, 
\begin{equation}
        \hat{\textbf{V}}_{t+1} = \textbf{V}_\text{t} -\Delta \text{t}\textit{\textbf{M}}^{-1}\frac{\delta \text{E}(\Gamma^\text{M})}{\delta \textbf{X}_{t}}, \, \,  \hat{\textbf{X}}_{\text{t}+1} = \textbf{X}_\text{t} + \Delta \text{t} \hat{\textbf{V}}_{t+1}
       \label{eq:Semi-Euler}
\end{equation}
However, based on experiment and natural deficiency from large-time step discretization, we found that this method could not capture high dynamic performance. We enhance the integration approach by incorporating predictive compensation. This enhancement is rooted in the concept of residual learning and is achieved through the adaptation of a graph neural network. Further details will be discussed in \ref{sec:integration_NN}.

==> revision_text/perception.tex <==
\section{DLO Tracking with Modeling}
\label{sec:tracking}

This section describes how we can use DEFORM to perform robust DLO tracking.
Notably, DEFORM enables us to deal with occlusions without requiring a frame-by-frame sensor update of the state of the DLO. 
In particular, this is possible due to our model accurately predicting the state of the DLO over long time horizons. 
As a result, we utilize a GMM model because it is independent of time. 
The state estimation approach is outlined in Algorithm~\ref{code:state estimation}. 
Additionally, Algorithm~\ref{code:DLO tracking} summarizes the perception pipeline that describes the tracking of DLOs with state estimation and initial state estimation using DEFORM.

\begin{algorithm}[t]
\caption{State Estimation with Presence of Occlusion} 
\label{code:state estimation}
% Initial State Estimation
% \begin{algorithmic}[1]
% \Require $\textbf{S}_1$ \Comment{RGB-D Camera}
% \If{Fully Observable}
% \State DLO Initialization $\leftarrow \text{GMM}(\textbf{S}_1)$
% \Else{}
% \State DLO Initialization $\leftarrow$ Guess
% \State DLO Initialization $\leftarrow \textbf{S}_1$ 
% \While {DLO not Reaches Static State}   
%          \State Execute DEFORM \Comment{\textbf{Algorithm. \ref{alg:long time horizon}, Assumption.\ref{assum: static initial}}}
% \EndWhile
% \State Return $\pred{X}{1}, \hat{\textbf{V}}_1 = \textbf{0}$
% \end{algorithmic}
\textbf{Inputs}: $\pred{X}{t+1}$\Comment{Algorithm. \ref{alg:long time horizon}}
\begin{algorithmic}[1]
% \While {$t = 1$ \textbf{to} $T$}
%     \State Execute DEFORM  \Comment{\textbf{Algorithm. \ref{alg:long time horizon}}}
% \EndWhile
% \State Return $\pred{X}{T+1}, \hat{\textbf{V}}_{T+1}$
\State $\textbf{S}_{T+1} \leftarrow \text{RGB-D Camera}$
\State $\tilde{\textbf{S}}_{T+1} \leftarrow \text{filter}(\pred{X}{t+1}, \textbf{S}_{T+1})$
\State Unoccluded $\pred{X}{t+1} \leftarrow $ Depth Matching($\tilde{\textbf{S}}_{T+1}$, $\pred{X}{t+1}$)
\State $n_{\tilde{}}+1$ groups $\leftarrow \text{DBSCAN}(\tilde{\textbf{S}}_{T+1})$
\For {each group}
\State GMM Number j $\leftarrow $ Match(Unoccluded $\pred{X}{t+1}$, group)
\State Mixture Center $\leftarrow$ GMM(group,  j)
\EndFor
% \State \textbf{\textcolor{blue}{for}} \Review{}{each group}{} \textbf{\textcolor{blue}{do}}
% \State\hspace{\algorithmicindent}\Review{}{GMM Number j $\leftarrow $ Match(Unoccluded $\pred{X}{t+1}$, group)}{}
% \State\hspace{\algorithmicindent}\Review{}{Mixture Center $\leftarrow$ GMM(group,  j)}{}
% \State \textbf{\textcolor{blue}{end for}}
% \State \textbf{\textcolor{blue}{for}} \Review{}{each $\pred{X}{t+1}$}{} \textbf{\textcolor{blue}{do}}
\For{each $\pred{X}{t+1}$}
% \State \hspace{\algorithmicindent}\textbf{\textcolor{blue}{if}} \Review{}{observed}{} \textbf{\textcolor{blue}{then}}
\If{Observed} 
\State Vertex $\leftarrow$ Associated Mixture Center
\Else
% \State \hspace{\algorithmicindent}\textbf{\textcolor{blue}{else}}
\State Vertex $\leftarrow$ Predicted Vertex
\EndIf{}
% \State \hspace{\algorithmicindent}\textbf{\textcolor{blue}{end if}}
% \State \textbf{\textcolor{blue}{end for}}
\EndFor
\State \Return: Vertices
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Tracking DLO with Modeling} 
\label{code:DLO tracking}
\textbf{Initial State Estimation}
\begin{algorithmic}[1]
\Require $\textbf{S}_1 \leftarrow $ RGB-D Camera
\State DLO Initial Guess $\leftarrow \textbf{S}_1$
\While{DLO not Static}
\State Execute DEFORM \Comment{Algorithm. \ref{alg:long time horizon}, Assumption.\ref{assum: static initial}}
\EndWhile
% \State \textbf{\textcolor{blue}{while}} \Review{}{DLO not Static}{} \textbf{\textcolor{blue}{do}}
%          \State \hspace{\algorithmicindent} \Review{}{Execute DEFORM \Comment{Algorithm. \ref{alg:long time horizon}, Assumption.\ref{assum: static initial}}}{}
% \textbf{\textcolor{blue}{end while}}
\State Return $\pred{X}{1}, \hat{\textbf{V}}_1 = \textbf{0}$
\end{algorithmic}
\textbf{Tracking DLO under Manipulation}
\begin{algorithmic}[1]
% \State \textbf{\textcolor{blue}{while}} \Review{}{Tracking DLO}{} \textbf{\textcolor{blue}{do}} 
% \State\hspace{\algorithmicindent}\textbf{\textcolor{blue}{while}} \Review{}{Predicting DLO}{} \textbf{\textcolor{blue}{do}}
% \State \hspace{\algorithmicindent} \hspace{\algorithmicindent} \Review{}{Execute DEFORM \Comment{Algorithm.\ref{alg:long time horizon}}}{}
% \State\hspace{\algorithmicindent}\textbf{\textcolor{blue}{end while}}
% \State \hspace{\algorithmicindent}\Review{}{State Estimation and Correction \Comment{Algorithm.\ref{code:state estimation}}}{}
% \State\textbf{\textcolor{blue}{end while}}
\While{Tracking DLO}
\While{Predicting DLO}
\State Execute DEFORM \Comment{Algorithm. \ref{alg:long time horizon}}
\EndWhile
\State State Estimation and Correction
\EndWhile
\end{algorithmic}
\end{algorithm}


% This section describes the perception pipeline that is used to verify the usefulness of modeling for robust DLO tracking and reducing perception frequency. 
% We assume prediction time to be extensively long so that the previous perception's geometry correlation with current perception can not be established efficiently. 
% Therefore, we keep GMM as it is to be time independent.

% \subsection{State Estimation}


\subsection{State Estimation in the Presence of Occlusions}
% \subsection{Prediction as Point Cloud Filter}
\label{section: filter}

% State estimation of DLO is crucial to initiate or refine prediction. 
Suppose that we are given access to an RGB-D sensor observing our DLO during manipulation and suppose that we translate these measurements at time step $t$ into a point cloud which we denote by  $\textbf{S}_t = \{s_t^1, s_t^m, \dots, s_t^M\} \Rdim{M}{3}$.
% \Yizhou{I made the change but it has overlap with related work...}

% \Zac{what makes this a problem?} \Zac{move this sentence up to after "If the DLO..."?} \Yizhou{problem: if set the number of mixtures in the GMM equal to the number of vertices of the DLO under occlusion, then unoccluded part will be overcrowed with vertices while occluded part does not have any vertices, which violates vertices distributions along DLOs.}
% let K to be the cluster number of point cloud, one can approximate DLO's keypoints as $\Tilde{\textbf{S}}_t = \text{GMM}(\textbf{S}_t, K)$  \cite[Section III.A]{Tomi2}. 
% When DLO is fully observable, K is set to be number of vertices n. 
% However, observe that $\Tilde{\textbf{S}}_t = \text{GMM}(\textbf{S}_t, K)$ does not have temporal correlation with previous observations. 
% Such temporal independence imposes challenge to address occlusion. 
% Recent literature \cite{cdcpd, cdcpd2, SPR, Tomi1, Tomi2} introduces local geometric regularization to leverage new observation $\textbf{S}_t$ and previous observation $\textbf{S}_{t-1}$. 
% Despite their success, geometric locality of those modeling methods require perception at each time step and could introduce unnecessary computational costs from perception. 
% To this end, we explore the possibility of relaxing the perception frequency while maintaining accuracy with our modeling.
To address the limitations of the algorithms discussed in Section \ref{sec:related_work}, we leverage our predictions generated by applying Algorithm \ref{alg:long time horizon} as follows.
% \Yizhou{I think it may make more sense to keep "our predictions generated by applying"}
We first filter the point cloud at time $t$ using our predicted data.
If any element of the point cloud is beyond some distance from our prediction, $\hat{\textbf{X}}_t$, then we remove it.
Let $\tilde{\textbf{S}}_t$ denote the remaining points in the point cloud.
Next, we detect which of the vertices of the DLO are unoccluded from the RGB-D sensor by checking if their predicted depth is close to their observed depth in the sensor.
Suppose the number of vertices that are unoccluded is $\tilde{n}$.

Once this is done, we apply DBSCAN to group $\tilde{\textbf{S}}_t$ into $\tilde{n}+1$ groups. 
Next, we associate each of the unoccluded vertices with one of the groups by finding the group to which its predicted location is smallest. 
We then take each group and perform GMM on the group with a number of mixtures equal to the number of vertices j that were associated with that group. 
Note, each mixture is associated with an unoccluded vertex of the DLO.
The new predicted location of the vertex generated by DEFORM is updated by setting the new vertex location equal to the mean of its associated mixture. % \Zac{is inextensibility checked here? if so, how?}
If a particular vertex was occluded, then its predicted location is left equal to its output from Algorithm~\ref{alg:long time horizon}.
% \Zac{I am confused by this section. do you start with a known state, then get a sensor measurement and compare that with the model prediction, and then update the model prediction somehow using the sensor measurement? at no point is it said where DEFORM is used. what is Alg 1 being used for? leverage vs augment? why are unoccluded vertices having GMM performed? what in here enables not doing a frame by frame update? is inextensibility still enforced after the update?}
% \Yizhou{"do you start with a known state, then get a sensor measurement and compare that with the model prediction, and then update the model prediction somehow using the sensor measurement?": yes
% "at no point is it said where DEFORM is used. what is Alg 1 being used for?": that is the reason why I was suggesting I think it may make more sense to keep "our predictions generated by applying". Alg 1 is to predict sequential states of DLOs. If perception is aquired at a point, the correponing prediction is used as a filter. "why are unoccluded vertices having GMM performed?" to correct unoccluded vertices. "what in here enables not doing a frame by frame update?" if the occlusion is persisting for a long time, the frame to frame update is not necessary and might have adversary effect. "is inextensibility still enforced after the update?" yes!}
% Raw observation of DLO with $\textbf{S}_t$ could be noisy and occluded. Prediction is applied to filter noise and occlusion. Naively applying GMM onto $\textbf{S}_t$ would be inapplicable. Therefore we apply prediction as filter as following.
% \begin{equation}
%     \Tilde{\textbf{S}}_t\in \{||\hat{\textbf{X}}_t - \textbf{S}_t||_2 \leq threshold\}
%     \label{eq:point cloud filter}
% \end{equation}
% Note that we differentiate filtered point cloud with observed point cloud with "$\sim$" (e.g., $\textbf{S}_t$ represents raw point and and $\Tilde{\textbf{S}}_t$ represents filtered point cloud.)

% \subsection{Leverage Perception and Prediction under Occlusion.}
% \label{sec: AdaptiveGMM}

% Applying GMM onto $\hat{\textbf{S}}_t$ with constant K under occlusion could introduce crowded vertices at observed point cloud and cause simulation inaccuracy. 
% Therefore, adaptive selection of K for observed point cloud is required. 
% Intuitively, point cloud under occlusion will spatially be divided into point cloud groups.
% We separate the group with DBSCAN \cite{DBSCAN}. Next, we assign center number onto each group sepererately with following: obtain predicted state $\hat{\textbf{X}}_t$'s depth by projecting through inverse of camera projection.
% Then, select out the non-occluded points $\Tilde{\textbf{X}}_t$ based mismatch between on $\hat{\textbf{X}}_t$'s depth and $\hat{\textbf{X}}_t$'s image location's perceived depth. 
% We then attribute $\hat{\textbf{X}}_t$ onto point cloud group by finding the summation of its distance costs \cite[cdist]{scipy} to each group. 
% Subsequently, each point cloud group uses number of attributed predicted points as number of cluster center. 
% Finally, observed prediction are leveraged with GMM's keypoint estimation, and keep unobserved prediction unchanged.

\subsection{Initial State Estimation under Occlusion}
\label{sec:initial_state}
Note that in many instances, it can be difficult to estimate the location of the vertices when the sensor turns on and the DLO is occluded.
Unfortunately, Algorithm~\ref{alg:long time horizon} and the state estimation algorithm from the previous subsection require access to a full initial state.
Fortunately, we can address this problem by making the following assumption:
\begin{assum}
When the sensor measurements begin, the DLO is static and is only subject to gravity and/or the manipulators which are holding its ends.
% when t=1, DLO is static and is only subjected to force from gravity and grippers.
\label{assum: static initial}
\end{assum}
Under the above assumption, we initialize the DLO using an initial guess that aligns with observed vertices.
This initial guess is then forward simulated using Algorithm~\ref{alg:long time horizon} repeatedly until the DLO reaches a static state.
This steady state is then used as the predicted state for all the vertices, including the occluded vertices. 
% \Zac{so the DLO can start in occlusion? if so this should be highlighted more. how well does this work?} \Yizhou{Yes. It is good suggestion. I could give out some quatitative data. Let's keep it in mind.}
% $\hat{\textbf{X}}_1$, that can be used in \eqref{eq:point cloud filter}.


% \begin{algorithm}
% \caption{Perception with Modeling} 
% \label{alg:inextensibility of PBD}
% \textbf{Initial Perception}: $\textbf{S}_1$
% \begin{algorithmic}[1]
% \State $\Tilde{\textbf{S}}_1\in \{||\hat{\textbf{X}}_1 - \textbf{S}_1||_2 \leq threshold\}$ \Comment{\secref{sec:initial_state}}
% \State Obtain $\textbf{X}_1$
% \Comment{\secref{sec:initial_state}, \secref{sec: AdaptiveGMM}}
% \Repeat
%     \For{$t = 1$ \textbf{to} $T-1$}
%         \State Execute \textbf{Algorithm. \ref{alg:long time horizon}}
%     \EndFor
%     \State \textbf{Perception:} $\textbf{S}_T$, Obtain $\textbf{X}_T$ \Comment{\secref{section: filter} \ref{sec: AdaptiveGMM}}
% \Until{Stop}
% \end{algorithmic}
% \end{algorithm}

==> revision_text/preliminaries.tex <==
\section{Preliminaries}
This section introduces the key components of DER while describing its limitations.
We conclude this section by describing how to simulate the behavior of a cable modeled as a Deformable Linear Object (DLO).
Note more details about DER can be found at \cite{originalDER} and in the appendix to this paper.
Throughout the rest of the document, let  $|\cdot|$ represents $||\cdot||_2$ and $\times$ denote the cross product between two vectors in $\R^3$.

\subsection{DLO Model}

We model the DLO using an indexed set of $n$ vertices at each time instance. 
The ground truth locations of vertex $i$ at time $t$ is denoted by $\timevertind{x}{i}{t} \in \R^3$ and the set of all $n$ vertices is denoted by $\timeind{X}{t}$. 
Let $\textit{\textbf{M}}^\text{i}\in \mathbb{R}^{3\times3}$ denote the mass matrix of vertex $i$.
The segments of the DLO are the lines between successive vertices, $\timevertind{e}{i}{t} = \timevertind{x}{i+1}{t} - \timevertind{x}{i}{t}$, and let $\timeind{E}{t}$ correspond to the set of all vertices at time $t$.

Our objective is to model the behavior of a DLO that is being controlled by a robot and as a result we make the following assumption:
\begin{assum}
    The first and last edge of the DLO are each held by a distinct end effector of a robot 
\end{assum}
\noindent Note this assumption is commonly made during wire manipulation \cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}.
Using this assumption, let the orientation and position of the two end effectors at time $t$ be denoted by $\vertindu_t \in \R^{12}$, which we refer to as the input.
Let $\textbf{U}_{1:\text{T}-1}$ denote the set of inputs applied between times $1$ and $\text{T}-1$, and let $\textbf{X}_{1:\text{T}} =\{\textbf{X}_1, \textbf{X}_2,\ldots, \textbf{X}_\text{T}\} \in \mathbb{R}^{\text{T} \times \text{n}\times 3}$ denote the associated trajectory of the DLO from times $1$ to $\text{T}$.

Let $\Delta_t$ denote the difference in time between successive elements of $\textbf{X}_{1:\text{T}}$.
Then let $\timeind{V}{t}  = (\timeind{X}{t} - \timeind{X}{t-1})/\Delta \text{t}$.
Finally note that we differentiate between ground truth elements and predicted elements by using ``hat'' (\textit{e.g.}, $\textbf{X}_{t}$ is the ground truth set of vertices at time $t$ and $\pred{X}{t}$ is the predicted set of vertices at time $t$).

\subsection{Modeling DLO with DER for Dual Manipulation}
\label{sec:DER}

\begin{figure}
    \centering
     \includegraphics[width=.5\textwidth]{figures/vertices.png}
     \caption{\textbf{replace with real world image}}
    \label{fig:primal-dual}
\end{figure}

DLOs primarily exhibit three distinct modes: bending, twisting, and inextensibility \Ram{need a citation here}.
Unfortunately, accurately modeling bending and twisting is challenging without introducing numerous additional parameters (e.g., stress and strain tensors) that can make it challenging to simulate the behavior of these models in real-time \cite{twistbendchallenge, twistbendchallenge2}.
To enforce inextensibility, it is typical to apply a large stretch stiffness, but this can introduce instabilities during simulation that can make using these models for prediction difficult. 
To address these challenges, (1) DER introduces a single scalar $\theta^\text{i}_{t} \in \R$ that accurately represents bending and twisting in $\R^3$ and (2) DER enforces inextensibility using a fast, stable projection method \cite[Section 4]{fast_proj}. 
Note, as this subsection's derivation is time-invariant, the time symbol $t$ is omitted for conciseness. 


\subsubsection{Reduced Frame Modeling Using the Bishop Frame} 

Typically, DLOs are modeled using a variety of coordinate frames called \emph{configuration frames} that are located at each vertex $i$.
These are denoted by $\Gamma^{i}$ for each $i \in \{1,\ldots,n-1\}$ and
are defined by three orthonormal vectors that correspond to the coordinate axes of the frame: $\bm{t}^\text{i}, \textbf{n}^\text{i},$ and $\textbf{b}^\text{i}$.
Note $\bm{t}^\text{i}=\textbf{e}^\text{i}/|\textbf{e}^\text{i}|$, $\vertind{n}{i}$ is the normal to $\vertind{t}{i}$, and $\vertind{b}{i}=\vertind{i}{i} \times \vertind{n}{i}$. 
To model the behavior of a DLO, one typically begins by computing the energy of the cable.
One can construct an approximation of the energy of a cable by computing the energy associated with bending and twisting at each of these different coordinate frames. 

To simplify this energy computation, DER begins by defining the \emph{Bishop frame}, $\Gamma^\text{i}_\text{B}$, which corresponds to a twist-free frame (i.e., it corresponds to the frame that is not rotated with respect to the frame centered at the previous edge, so the energy associated with twisting is minimized in this frame). 
To formalize this notion, suppose the Bishop frame has coordinate axes $\textbf{t}^\text{i}, \textbf{w}_1^\text{i},$ and $\textbf{w}_2^\text{i}$ that are formally defined in the Appendix for convenience.
Let $\theta^\text{i}$ correspond to the rotation about $\vertind{t}{i}$ starting from the Bishop frame to generate a coordinate frame $\Gamma^\text{i}_\text{B}(\theta^i)$, which has coordinate axis $\textbf{t}^\text{i}, \textbf{m}_1^\text{i},$ and $\textbf{m}_2^\text{i}$ where:
\begin{align}
    \textbf{m}_1^\text{i}&=\text{cos}\theta^\text{i}\cdot \textbf{w}_1^\text{i} + \text{sin}\theta^\text{i}\cdot \textbf{w}_2^\text{i},\\
    \textbf{m}_2^\text{i}&=-\text{sin}\theta^\text{i}\cdot \textbf{w}_1^\text{i} + \text{cos}\theta^\text{i}\cdot \textbf{w}_2^\text{i}.
\end{align}
Note that  $\Gamma^\text{i}_\text{B} = \Gamma^\text{i}_\text{B}(0)$.
The Bishop frame satisfies the following lemma whose proof can be found in \Ram{please reference a specific paper's proof of this lemma}:
\begin{lem}
\label{lem:bishop_twist}
Let  $\overline{\textbf{B}}_\text{i} \in \mathbb{R}^{2 \times 2}$ denote the bending modulus of vertex $i$ which is a material property of the cable.
    Let $E_\text{twist}(\Gamma^\text{i}_\text{B}(\theta^\text{i}),\overline{\textbf{B}}_\text{i})$ denote the twisting energy of $\Gamma^\text{i}_\text{B}(\theta^i)$. 
    Then $E_\text{twist}(\Gamma^\text{i}_\text{B}(\theta^\text{i}),\overline{\textbf{B}}_\text{i})\geq E_\text{twist}(\Gamma^\text{i}_\text{B}(0),\overline{\textbf{B}}_\text{i})$ for all $\theta^i$.
\end{lem}
Similarly one can start from the Bishop frame, rotate it by $\theta^i$, and project it on the curvature binormal vector to construct the \emph{Curvature Binormal Frame}, $\Gamma^\text{i}_\text{C}(\theta^i)$. 
For conciseness, we leave the derivation of this frame to the Appendix \Ram{make sure this is done}. 
However, one can prove the following result related to the bending energy using the Curvature Binormal Frame:
\begin{lem}
\label{lem:bishop_bend}
    Let $E_\text{bend}(\Gamma^\text{i}_\text{C}(\theta^i))$ denote the bending energy of $\Gamma^\text{i}_\text{C}(\theta^i)$. 
    Then $E_\text{bend}(\Gamma^\text{i}_\text{C}(0))\geq E_\text{bend}(\Gamma^\text{i}_\text{C}(\theta^\text{i}))$ for all $\theta^i$.
\end{lem}
Lemmas \ref{lem:bishop_twist} and \ref{lem:bishop_bend} allow one to compute the energy of a DLO that arises due to bending and twisting by using Bishop and Curvature Binormal Frame rather than working directly in the configuration frame. 
\Ram{will we present the formulas for the energy somewhere and do we want to say that they are convex functions of $\theta$ or something?}
As we show in Section \ref{sec:integration}, once we compute the energy of the DLO, then we can simulate its behavior.

\subsubsection{Inextensibility Enforcement}
During simulation, the DLO's length may change, but this is not a typical property of most cables.
To ensure that the length of the DLO does not change during simulation, DER perform projection of a computed solution to ensure that the following constraint is satisfied:
\begin{equation}
    \textbf{e}_\text{i} \cdot \textbf{e}_\text{i} - \overline{\textbf{e}}_\text{i}\cdot\overline{\textbf{e}}_\text{i} = 0
\label{eq:inextensibility}
\end{equation}
where $\overline{\textbf{e}}_\text{i}$ denotes the undeformed edge. 
Unfortunately to ensure stability while performing simulation, this method requrest it to use small step sizes. 
As a result, in this paper we adopt a constraint solver based on position-based dynamics(PBD) \cite{PBD} that is described in Section\ref{sec:inextensiblity methodology}. 

\subsection{DLO Simulation Using DER}
\label{sec:integration}

To simulate the behavior of the DLO, we use DER to compute the total energy of the cable. 
Once that total energy is computed, one can apply state of the art ordinary differential equation solvers to simulate the behavior of the system.
However, to do this we need to assume that the cable reaches an equilibrium state between each simulation time step:
\begin{assum}
    The Bishop and Curvature Binormal Frame reach an equilibrium state at each time step. 
    As a result, at each time step $t$ one can compute 
    \begin{equation}
        \symbind{\theta}{i}^*_t = \underset{\theta^i_t}{\arg\min} \left(E_\text{twist}(\symbind{\Gamma}{i}_\text{B}(\theta^\text{i}_t)) + E_\text{bend}(\symbind{\Gamma}{i}_\text{C}(\theta^\text{i}_t)) \right)
        \label{eq:opt_theta}
    \end{equation}
\end{assum}

For conciseness, let $\theta_t^*$ represent all of the rotational parameters associated with the Bishop and Curvature Binormal Frames for a particular $\timeind{X}{t}$. 
Note that $\theta^*_\text{t}$ is a function of $\timeind{X}{t}$. 
As a result, the total energy of the cable at time step $t$ is:
\begin{equation}
    \text{E}(\textbf{X}_t) = \sum^{n-1}_{i=2} \left(\text{E}_{\text{twist}}(\Gamma_\text{B}^\text{i}(\symbind{\theta}{i}_t^*)) + \text{E}_{\text{bend}}(\Gamma_\text{C}^{i}(\symbind{\theta}{i}_t^*))\right) 
    \label{eq:energy}
\end{equation}
This representation enables us to perform simulation as we describe next.


Because the negative of the derivative of the total (potential) energy of the cable is equal to the force into the system, one can apply derive the following equation of motion from Newton's Second Law:
\begin{equation}
       \textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{d\text{E}(\textbf{X}_t)}{d \textbf{X}_{t}}
       \label{eq:Integration}
\end{equation}
One can numerically integrate this formula to predict the velocity and position:
\begin{align}
        \hat{\textbf{V}}_{t+1} &= \hat{\textbf{V}}_\text{t}-\Delta_\text{t}m^{-1}\frac{d\text{E}(\textbf{X}_t)}{d \textbf{X}_{t}}, \\  
        \hat{\textbf{X}}_{\text{t}+1} &= \hat{\textbf{X}}_\text{t} + \Delta_\text{t}\hat{\textbf{V}}_{t+1}.
       \label{eq:Semi-Euler}
\end{align}
However, if the time step is large, it can be challenging to simulate these models accurately.
To address this challenge in \secref{sec:Differentiable DER} we develop a differentiable simulation model that enables to apply residual learning to perform predictive compensation during integration as is described in \secref{sec:integration_NN}.
% However, based on experiment and natural deficiency from large-time step discretization, we find that this method cannot capture high dynamic performance. 
% We enhance the integration approach by incorporating predictive compensation. 
% This enhancement is rooted in the concept of residual learning and is achieved through the adaptation of a graph neural network. 
% Further details will be discussed in \secref{sec:integration_NN}.
% ; however, note that our goal is to eventually perform differentiable simulation to allow for auto-tuning certain model parameters which is described in more detail in \secref{sec:Differentiable DER}.

% \subsection{Long Time Horizon Prediction for DLO}

% Following assumptions are made to setup a prediction framework.
% \begin{assum}
%     first two states $\timeind{X}{1}, \timeind{X}{2}$ are fully observable. 
% \end{assum}
% Satisfying this assumption is essential for the initialization of iterative prediction. However, when perception is heavily occluded at the initial state, meeting above assumption can be challenging. Details will be discussed in \secref{section: Estimation}
% \begin{assum}
% End edges of wire are coupled with grippers such that $\textbf{u}_\text{t}=\{\timevertind{x}{1}{t+1}, \timevertind{x}{2}{t+1}, \timevertind{x}{n-1}{t+1}, \timevertind{x}{n}{t+1}\}$. $\textbf{u}_\text{t}$ can be approximated through inverse kinematics or other perception system.
% \end{assum}
% Above assumption commonly made and well-studied in wire manipulation among literature\cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}. It provides accessibility and controllability to wire edges.

%  \Ram{use an assumption environment like in the file I shared with you....} 
% \Ram{what does this mean?}. With above assumptions, denote $F$ as a general modeling function, long-time horizon inference is propagated through iterative prediction as shown in the \textbf{Algorithm} \ref{alg:long time horizon}. Note ground truth is not accessible during the iteration, and all predicted intermediate and final states of the wire will be used for evaluation. 
% \begin{algorithm}[t]
% \caption{Long Time Horizon Prediction } 
% \label{alg:long time horizon}
% \textbf{Require:} $\textbf{X}_{1:\text{T}}, \textbf{U}_{2:\text{T-1}}$ \Comment{True States and Inputs}\\
% \textbf{Initialization} at t = 2: 
% \begin{algorithmic}[1]
% \State $\textbf{V}_2 = (\textbf{X}_2 - \textbf{X}_1)/\Delta \text{t}$ \Comment{Initial Velocity Estimation } 
% \State $\pred{X}{3} = F(\textbf{u}_2, \textbf{X}_2, \textbf{V}_2)$   \Comment{First Update}
% \State $\pred{V}{3} = (\pred{X}{3} - \textbf{X}_2)/\Delta \text{t}$ \Comment{Velocity Update}
% \State {Iterative Update: $\text{T} \gg \Delta \text{t}$ \Ram{not sure why you need this condition...I think you are just running a for loop? Also isn't this just a single algorithm, why does the line number change halfway thru? Is this supposed to be two algorithms? Then call them two algorithms?}} \Yizhou{I was trying to show it is long time horizon but I can delete this line.}
% \For{$\text{t} \gets 3 \textrm{ to } \text{T}-1$} 
%      \State $\pred{X}{t+1} = F(\textbf{u}_\text{t}, \pred{X}{t}, \pred{V}{t})$
%      \State $\pred{V}{t+1} = (\pred{X}{t+1} - \pred{X}{t})/\Delta t$
% \EndFor
% \State \Return $\pred{X}{3:T}, \, |\pred{X}{3:T} - \timeind{X}{3:T}|$ \Comment{Prediction and Loss}
% \end{algorithmic}
% \end{algorithm}


% \subsection{Integration for DLO Simulation}
% \label{sec:integration}
% Notice that $\theta^*_\text{t}$ is a function of $\timeind{X}{t}$. For conciseness, based on \Eqref{eq:energy}, we note equation of motion as follows: 
% \begin{equation}
%        \textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\delta \text{E}(\Gamma^\text{M}(\timeind{X}{t}))}{\delta \textbf{X}_{t}}
%        \label{eq:Integration}
% \end{equation}
% As DER is not an analytical modeling frame. Solving  \Eqref{eq:Integration} requires numerical integration. DER\cite{originalDER} choose the method to be Semi-Euler method\cite{implicit-euler}, which has the same computational cost while having better tracking performance compared to Euler's method, as shown in the following, 
% \begin{equation}
%         \hat{\textbf{V}}_{t+1} = \textbf{V}_\text{t} -\Delta \text{t}m^{-1}\frac{\delta \text{E}(\Gamma^\text{M}(\textbf{X}_{t}))}{\delta \textbf{X}_{t}}, \, \,  \hat{\textbf{X}}_{\text{t}+1} = \textbf{X}_\text{t} + \Delta \text{t} \hat{\textbf{V}}_{t+1}
%        \label{eq:Semi-Euler}
% \end{equation}
% However, based on experiment and natural deficiency from large-time step discretization, we find that this method cannot capture high dynamic performance. We enhance the integration approach by incorporating predictive compensation. This enhancement is rooted in the concept of residual learning and is achieved through the adaptation of a graph neural network. Further details will be discussed in \secref{sec:integration_NN}.

% \subsection{Long Time Horizon Prediction for DLO}
% Following assumptions are made to setup a prediction framework.
% \begin{assum}
%     first two states $\timeind{X}{1}, \timeind{X}{2}$ are fully observable. 
% \end{assum}
% Satisfying this assumption is essential for the initialization of iterative prediction. However, when perception is heavily occluded at the initial state, meeting above assumption can be challenging. Details will be discussed in \secref{section: Estimation}
% \begin{assum}
% End edges of wire are coupled with grippers such that $\textbf{u}_\text{t}=\{\timevertind{x}{1}{t+1}, \timevertind{x}{2}{t+1}, \timevertind{x}{n-1}{t+1}, \timevertind{x}{n}{t+1}\}$. $\textbf{u}_\text{t}$ can be approximated through inverse kinematics or other perception system.
% \end{assum}
% Above assumption commonly made and well-studied in wire manipulation among literature\cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}. It provides accessibility and controllability to wire edges.

%  \Ram{use an assumption environment like in the file I shared with you....} 
% \Ram{what does this mean?}. With above assumptions, denote $F$ as a general modeling function, long-time horizon inference is propagated through iterative prediction as shown in the \textbf{Algorithm} \ref{alg:long time horizon}. Note ground truth is not accessible during the iteration, and all predicted intermediate and final states of the wire will be used for evaluation. 
% \begin{algorithm}
% \caption{Long Time Horizon Prediction } 
% \label{alg:long time horizon}
% \textbf{Require:} $\textbf{X}_{1:\text{T}}, \textbf{U}_{2:\text{T-1}}$ \Comment{True States and Inputs}\\
% \textbf{Initialization} at t = 2: 
% \begin{algorithmic}[1]
% \State $\textbf{V}_2 = (\textbf{X}_2 - \textbf{X}_1)/\Delta \text{t}$ \Comment{Initial Velocity Estimation } 
% \State $\pred{X}{3} = F(\textbf{u}_2, \textbf{X}_2, \textbf{V}_2)$   \Comment{First Update}
% \State $\pred{V}{3} = (\pred{X}{3} - \textbf{X}_2)/\Delta \text{t}$ \Comment{Velocity Update}
% \State {Iterative Update: $\text{T} \gg \Delta \text{t}$ \Ram{not sure why you need this condition...I think you are just running a for loop? Also isn't this just a single algorithm, why does the line number change halfway thru? Is this supposed to be two algorithms? Then call them two algorithms?}} \Yizhou{I was trying to show it is long time horizon but I can delete this line.}
% \For{$\text{t} \gets 3 \textrm{ to } \text{T}-1$} 
%      \State $\pred{X}{t+1} = F(\textbf{u}_\text{t}, \pred{X}{t}, \pred{V}{t})$
%      \State $\pred{V}{t+1} = (\pred{X}{t+1} - \pred{X}{t})/\Delta t$
% \EndFor
% \State \Return $\pred{X}{3:T}, \, |\pred{X}{3:T} - \timeind{X}{3:T}|$ \Comment{Prediction and Loss}
% \end{algorithmic}
% \end{algorithm}


% To formulate reduced coordinate modeling, $\theta^\text{i}$ is introduced to measures the rotation about $\vertind{t}{i}$ from Bishop frame $\Gamma^\text{i}_\text{B}: {\{\textbf{t}^\text{i}, \textbf{v}_1^\text{i}, \textbf{v}_2^\text{i}\}}$ relative to material frame material frame $\Gamma^\text{i}_\text{M}:\{\boldsymbol{\textbf{t}}^\text{i}, \textbf{m}_1^\text{i}, \textbf{m}_2^\text{i}\}$ with following equation.
% \begin{equation}
%     \textbf{m}_1^\text{i}=\text{cos}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{sin}\theta^\text{i}\cdot \textbf{v}_2^\text{i}, \textbf{m}_2^\text{i}=-\text{sin}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{cos}\theta^\text{i}\cdot \textbf{v}_2^\text{i}
% \end{equation}
% Bishop frame is referred as twist-free frame according to following lemma:
% \begin{lem}
%     Let $E_\text{twist}(\Gamma^\text{i}(\theta^\text{i}))$ denote twisting energy of $\Gamma^\text{i}$. $\forall \theta^\text{i} \neq 0, E_\text{twist}(\Gamma^\text{i}_\text{M}(\theta^\text{i}))\geq E_\text{twist}(\Gamma^\text{i}_\text{M}(\theta^\text{i}=0)=\Gamma^\text{i}_\text{B})$
% \end{lem}
% Such property is critical as it allows the material frame to use Bishop frame as a reference frame (energy-minimized frame) to capture twisting efficiently. Importantly, bending energy of  material frame has following property.
% \begin{lem}
%     Let $E_\text{bend}(\symbind{\Gamma}{i}(\vertind{e}{i-1}, \vertind{e}{i}, \theta^\text{i})$ denote bending energy of $\symbind{\Gamma}{i}$. $\forall \theta^\text{i} \neq 0, E_\text{bend}(\Gamma^\text{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i},0))\geq E_\text{bend}(\symbind{\Gamma}{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i},\theta^\text{i}))$
% \end{lem}
% Lemma 1 and Lemma 2 allow $\theta^\text{i}$ to distribute twisting and bending energy within a bounded material frame energy. The weight of each is based on quasistatic treatment with the following assumption.
% \begin{assum}
%     The material frame always reaches an equilibrium state before simulating the next step, as $E_\text{twist}(\symbind{\Gamma}{i}_\text{M}(\theta^\text{i})) + E_\text{bend}(\symbind{\Gamma}{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i}, \theta^\text{i}))$ is bounded, $(\symbind{\theta}{i})^*$ can always be solved with following:
%     \begin{equation}
%         (\symbind{\theta}{i})^* = \underset{\theta^i}{\arg\min}(E_\text{twist}(\symbind{\Gamma}{i}_\text{M}(\theta^\text{i})) + E_\text{bend}(\symbind{\Gamma}{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i},\theta^\text{i})))
%         \label{eq:opt_theta}
%     \end{equation}
% \end{assum}
% Final energy is expressed as following:
% \begin{equation}
%     \text{E}(\Gamma^\text{M}(\theta^*), \textbf{E}) = \sum^{n-1}_{i=2}\text{E}_{\text{twist}}(\Gamma_\text{M}^\text{i}((\symbind{\theta}{i})^*)) + \text{E}_{\text{bend}}(\Gamma_\text{M}^{i}(\vertind{e}{i-1}, \vertind{e}{i}, (\symbind{\theta}{i})^*)) 
%     \label{eq:energy}
% \end{equation}
% Such energy formulation in reduced coordinates facilitates computation efficiency while managing to perform bending and twisting. Despite its success, notice we want to build a differentiable simulation that enables parameter auto-tuning. However, solving of Eq.\ref{eq:opt_theta} poses challenge to obtain gradients, which will be discussed in \secref{sec:Differentiable DER}.


% \subsection{Integration for DLO Simulation}
% \label{sec:integration}
% Notice that $\theta^*_\text{t}$ is a function of $\timeind{X}{t}$. For conciseness, based on \Eqref{eq:energy}, we note equation of motion as follows: 
% \begin{equation}
%        \textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\delta \text{E}(\Gamma^\text{M}(\timeind{X}{t}))}{\delta \textbf{X}_{t}}
%        \label{eq:Integration}
% \end{equation}
% As DER is not an analytical modeling frame. Solving  \Eqref{eq:Integration} requires numerical integration. DER\cite{originalDER} choose the method to be Semi-Euler method\cite{implicit-euler}, which has the same computational cost while having better tracking performance compared to Euler's method, as shown in the following, 
% \begin{equation}
%         \hat{\textbf{V}}_{t+1} = \textbf{V}_\text{t} -\Delta \text{t}m^{-1}\frac{\delta \text{E}(\Gamma^\text{M}(\textbf{X}_{t}))}{\delta \textbf{X}_{t}}, \, \,  \hat{\textbf{X}}_{\text{t}+1} = \textbf{X}_\text{t} + \Delta \text{t} \hat{\textbf{V}}_{t+1}
%        \label{eq:Semi-Euler}
% \end{equation}
% However, based on experiment and natural deficiency from large-time step discretization, we find that this method cannot capture high dynamic performance. We enhance the integration approach by incorporating predictive compensation. This enhancement is rooted in the concept of residual learning and is achieved through the adaptation of a graph neural network. Further details will be discussed in \secref{sec:integration_NN}.

% \subsection{Long Time Horizon Prediction for DLO}
% Following assumptions are made to setup a prediction framework.
% \begin{assum}
%     first two states $\timeind{X}{1}, \timeind{X}{2}$ are fully observable. 
% \end{assum}
% Satisfying this assumption is essential for the initialization of iterative prediction. However, when perception is heavily occluded at the initial state, meeting above assumption can be challenging. Details will be discussed in \secref{section: Estimation}
% \begin{assum}
% End edges of wire are coupled with grippers such that $\textbf{u}_\text{t}=\{\timevertind{x}{1}{t+1}, \timevertind{x}{2}{t+1}, \timevertind{x}{n-1}{t+1}, \timevertind{x}{n}{t+1}\}$. $\textbf{u}_\text{t}$ can be approximated through inverse kinematics or other perception system.
% \end{assum}
% Above assumption commonly made and well-studied in wire manipulation among literature\cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}. It provides accessibility and controllability to wire edges.

%  \Ram{use an assumption environment like in the file I shared with you....} 
% \Ram{what does this mean?}. With above assumptions, denote $F$ as a general modeling function, long-time horizon inference is propagated through iterative prediction as shown in the \textbf{Algorithm} \ref{alg:long time horizon}. Note ground truth is not accessible during the iteration, and all predicted intermediate and final states of the wire will be used for evaluation. 
% \begin{algorithm}
% \caption{Long Time Horizon Prediction } 
% \label{alg:long time horizon}
% \textbf{Require:} $\textbf{X}_{1:\text{T}}, \textbf{U}_{2:\text{T-1}}$ \Comment{True States and Inputs}\\
% \textbf{Initialization} at t = 2: 
% \begin{algorithmic}[1]
% \State $\textbf{V}_2 = (\textbf{X}_2 - \textbf{X}_1)/\Delta \text{t}$ \Comment{Initial Velocity Estimation } 
% \State $\pred{X}{3} = F(\textbf{u}_2, \textbf{X}_2, \textbf{V}_2)$   \Comment{First Update}
% \State $\pred{V}{3} = (\pred{X}{3} - \textbf{X}_2)/\Delta \text{t}$ \Comment{Velocity Update}
% \State {Iterative Update: $\text{T} \gg \Delta \text{t}$ \Ram{not sure why you need this condition...I think you are just running a for loop? Also isn't this just a single algorithm, why does the line number change halfway thru? Is this supposed to be two algorithms? Then call them two algorithms?}} \Yizhou{I was trying to show it is long time horizon but I can delete this line.}
% \For{$\text{t} \gets 3 \textrm{ to } \text{T}-1$} 
%      \State $\pred{X}{t+1} = F(\textbf{u}_\text{t}, \pred{X}{t}, \pred{V}{t})$
%      \State $\pred{V}{t+1} = (\pred{X}{t+1} - \pred{X}{t})/\Delta t$
% \EndFor
% \State \Return $\pred{X}{3:T}, \, |\pred{X}{3:T} - \timeind{X}{3:T}|$ \Comment{Prediction and Loss}
% \end{algorithmic}
% \end{algorithm}



% The bishop frame is defined as following:
% \begin{defn}
%     \label{def: Bishop}
%      Denote $\bm{v^\text{i+1}} = R_{\text{q}^\text{i}}(\bm{v^\text{i}}), \, \text{q}^\text{i}=(\text{q}_0^\text{i}, \textbf{q}^\text{i})$ as quaternion rotation that rotates $\bm{v^\text{i}}$ around axial vector $\textbf{q}^\text{i}$ with magnitude $\text{q}_0^\text{i}$. Let $\phi^\text{i}$ denote the turning angle between $\vertind{e}{i}$ and $\vertind{e}{i+1}$. Given 
% \begin{equation}
% \textbf{t}^{\text{i}+1} =R_{\text{q}^\text{i}}(\textbf{t}^\text{i}),\, \textbf{n}_1^{\text{i}+1} \label{eq:parallel transfort1} =R_{\text{q}^\text{i}}(\textbf{n}_1^\text{i})
% \end{equation}  
% \begin{equation}
% \text{q}_0^\text{i} = \text{cos}(\phi^\text{i}/2), \, \textbf{q}^\text{i} = \text{sin}(\phi^\text{i}/2)(\textbf{t}^\text{i} \times \textbf{t}^{\text{i}+1})
% \label{eq:parallel transfort2}    
% \end{equation}
% A frame that is transported with above equations is Bishop frame $\Gamma^\text{i}_\text{B}: {\{\textbf{t}, \textbf{v}_1, \textbf{v}_2\}}$.
% % \end{defn}
% \begin{defn}
%     \label{def: material frame}
%     Let a rotation angle $\vertind{$\theta$}{i}$ that represents rotation from Bishop frame to material frame $\Gamma^\text{i}_\text{M}:{\{\boldsymbol{\textbf{t}}^\text{i}, \textbf{m}_1^\text{i}, \textbf{m}_2^\text{i}}\}$ about $\vertind{t}{i}$ with the following equation.
% \begin{equation}
%     \textbf{m}_1^\text{i}=\text{cos}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{sin}\theta^\text{i}\cdot \textbf{v}_2^\text{i}, \textbf{m}_2^\text{i}=-\text{sin}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{cos}\theta^\text{i}\cdot \textbf{v}_2^\text{i}
% \end{equation}


==> revision_text/preliminaries_new.tex <==
\section{Preliminaries}
\label{Appendix: DER}
% \begin{wrapfigure}{R}{0.45\textwidth} 
%     \vspace*{-1.0cm}
%     \centering
%      \includegraphics[width=0.42\textwidth]{figures/DlO.PNG}
%      \caption{A Deformable Linear Object (DLO) model that describes the notation used throughout the paper.}
%     \label{fig:DLO}
%     \vspace*{-1.1cm}
% \end{wrapfigure}
This section introduces the key components of DER models while describing their limitations.
Note that more details about DER can be found at \cite{originalDER}. \Revise{We also introduce existing state estimation algorithms of DLOs and discuss potential improvements.}{}% Throughout the rest of the document, let  $|\cdot|$ represents $||\cdot||_2$ and $\times$ denote the cross product between two vectors in $\R^3$.
 \subsection{Deformable Linear Object (DLO) Model}
To model a DLO, we separate the DLO into an indexed set of $n$ vertices at each time instance. 
The ground truth locations of vertex $i$ at time $t$ is denoted by $\timevertind{x}{i}{t} \in \R^3$ and the set of all $n$ vertices is denoted by $\timeind{X}{t}$ as illustrated in Figure \ref{fig:DLO}. 
Let $\textit{\textbf{M}}^\text{i}\in \mathbb{R}^{3\times3}$ denote the mass matrix of vertex $i$.
A segment, or edge, in the DLO is the line between successive vertices, $\timevertind{e}{i}{t} = \timevertind{x}{i+1}{t} - \timevertind{x}{i}{t}$.
Let $\timeind{E}{t}$ correspond to the set of all edges at time $t$.
Our objective is to model the dynamic behavior of a DLO that is being controlled by a robot and as a result we make the following assumption:
\begin{assum}
    The first and last edge of the DLO are each held by a distinct end effector of a robot 
    \label{assum:grasp condition}
\end{assum}
Note this assumption is commonly made during DLO manipulation \cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}. Using this assumption, let the orientation and position of the two end effectors at time $t$ be denoted by $\vertindu_t \in \R^{12}$, which we refer to as the input.
Let $\textbf{U}_{1:\text{T}-1}$ denote the set of inputs applied between times $t=1$ and $t=\text{T}-1$, and let $\textbf{X}_{1:\text{T}} =\{\textbf{X}_1, \textbf{X}_2,\ldots, \textbf{X}_\text{T}\} \in \mathbb{R}^{\text{T} \times \text{n}\times 3}$ denote the associated trajectory of the DLO from times $t=1$ to $t=\text{T}$.

Let $\Delta_t$ denote the difference in time between successive elements of $\textbf{X}_{1:\text{T}}$.
Then, the velocity of the vertices of the DLO can be denoted as $\timeind{V}{t}  = (\timeind{X}{t} - \timeind{X}{t-1})/\Delta \text{t}$.
Finally, note that we distinguish between ground truth elements and predicted elements by using the circumflex symbol (\textit{e.g.}, $\textbf{X}_{t}$ is the ground truth set of vertices at time $t$ and $\pred{X}{t}$ is the predicted set of vertices at time $t$).

\subsection{Modeling DLO with DER for Dual Manipulation}
\label{sec:DER}

DLOs primarily exhibit three distinct modes: bending, twisting, and stretching \cite{originalDER}. 
% \Zac{is modes the word used by the cited paper? I feel like deformation modes makes sense for the first two, but not inextensibility. maybe change inextensibility to stretching.} \Yizhou{I think it might be ok to keep this? otherwise we need to have another sentence to connect stretching and inextensibility?}
In this paper, we focus on DLOs that are inextensible, and therefore do not experience stretching.
Accurately modeling the bending and twisting modes of a DLO is challenging without introducing a large number of parameters.
Unfortunately, the behavior of a model with large numbers of parameters is challenging to simulate in real-time \cite{twistbendchallenge, twistbendchallenge2}.
To enforce inextensibility, it is typical to apply a large stretch stiffness, but this can introduce instabilities during simulation, making these models difficult to use for prediction.
To address these challenges, (1) DER introduces a single scalar $\theta^\text{i}_{t} \in \R$ that accurately represents bending and twisting in $\R^3$ and (2) DER enforces inextensibility using a fast, stable projection method \cite[Section 4]{fast_proj}. 

\subsection{Potential Energy to Equations of Motion} 

A DLO can be modeled using DER by first introducing a family of frames that are collocated with each of the vertices. 
In particular, each frame's relationship with the prior frame is parameterized by $\theta^\text{i}_t \in \R$.
An explanation for why a single scalar is sufficient to describe this rotation can be found in \cite[Section 4.2]{originalDER}.
If one is given $\textbf{X}_t$, then one can compute $\theta^\text{i}_t$.
As a result, we write $\bm{\theta}_t(\textbf{X}_t)$ to denote the vector of all $\theta^\text{i}_t$ at a time $t$.
Note, we explain how to compute $\bm{\theta}_t(\textbf{X}_t)$ before the end of this section.

Using this representation, DER is able to accurately approximate the potential energy of the DLO that arises due to bending or twisting. 
This potential energy is a function of the material properties of each vertex of the DLO (i.e., their mass, bending modulus, and twisting modulus) and the configuration of the DLO.
If we let $\bm{\alpha}$ denote the vector of the material properties of each vertex of the DLO, then one can write down the potential energy of a particular configuration of the DLO as $P(\textbf{X}_t, \bm{\theta}_t(\textbf{X}_t),\bm{\alpha})$ \cite[Section 4.2]{originalDER}.

Once the potential energy expression is derived, then the restorative force experienced during deformation is equal to the negative of the gradient of the potential energy expression with respect to the vertices. Therefore, the equation of motion of the DLO is:
\begin{equation}
       \textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\partial P(\textbf{X}_t, \bm{\theta}_t(\textbf{X}_t),\bm{\alpha})}{\partial  \textbf{X}_{t}}
       \label{eq:Integration}
\end{equation}
One can numerically integrate this formula to predict the velocity and position by applying the Semi-Implicit Euler method:
\begin{align}
        \hat{\textbf{V}}_{t+1} &= \hat{\textbf{V}}_\text{t}-\Delta_\text{t}M^{-1}\frac{\partial P(\hat{\textbf{X}}_t, \bm{\theta}_t(\hat{\textbf{X}}_t),\bm{\alpha})}{\partial \textbf{X}_{t}}, \label{eq:Semi-Euler1}\\  
        \hat{\textbf{X}}_{\text{t}+1} &= \hat{\textbf{X}}_\text{t} + \Delta_\text{t}\hat{\textbf{V}}_{t+1}.
       \label{eq:Semi-Euler2}
\end{align}

One can use \eqref{eq:Semi-Euler1}-\eqref{eq:Semi-Euler2} with state-of-the-art ODE solvers to simulate the behavior of the DER model of a DLO.
However, computing the gradient of the potential energy requires an expression for $\bm{\theta}_t(\textbf{X}_t)$. 
To construct such an expression, DER assumes that the DLO reaches an equilibrium state between each simulation time step:
\begin{assum}
    Between each step of the simulation, the DLO reaches an equilibrium state. 
    As a result, at each time step $t$, one can compute
    \begin{equation}
        \bm{\theta}^*_t(\textbf{X}_t) = \argmin_{\bm{\theta}_t} P(\textbf{X}_t, \bm{\theta}_t,\bm{\alpha})
        \label{eq:opt_theta}
    \end{equation}
\end{assum}
To summarize, at each integration time step, one must solve \eqref{eq:opt_theta} to evaluate the dynamics. 
There are several factors which make simulating this model  quickly and accurately challenging.
First, it may be difficult to accurately estimate the material properties of an arbitrary DLO before simulating the model. 
In \secref{sec:Differentiable DER}, we illustrate how to make the DER model differentiable so that one can estimate the material properties from real-world data while simulating the model.
Second, there is an undesirable tradeoff between choosing a larger time step to achieve real-time prediction and the accuracy of that prediction.
In \secref{sec:integration_NN}, we apply residual learning to perform predictive compensation during integration which enables rapid simulation of the model without sacrificing accuracy.


\subsubsection{Inextensibility Enforcement}
During simulation, the DLO's length may change due to numerical errors, but this is undesirable when modeling DLOs like cables and ropes, which are inextensible.
To ensure that the length of the DLO does not change during simulation, DER methods project a computed solution onto a constraint set that ensures that the DLO's length does not change.
% \begin{equation}
%     \textbf{e}_\text{i} \cdot \textbf{e}_\text{i} - \overline{\textbf{e}}_\text{i}\cdot\overline{\textbf{e}}_\text{i} = 0
% \label{eq:inextensibility}
% \end{equation}
% where $\overline{\textbf{e}}_\text{i}$ denotes the undeformed edge. 
However, this projection operation can introduce instabilities during simulation because it does not ensure that momentum is conserved during motion.
This papers adopts a constraint solver based on a PBD model \cite{PBD}, which is described in Section \ref{sec:inextensiblity methodology}, to enforce inextensiblity while conserving momentum.
This improves the accuracy of prediction when compared to classical methods. 

% \begin{wrapfigure}{R}{0.6\textwidth}
%       \vspace*{-0.65cm}
%     \begin{minipage}{0.6\textwidth}
%       \begin{algorithm}[H]
% \caption{One Step Prediction} 
% \label{alg:long time horizon}
% \textbf{Inputs}: $\pred{X}{t}, \pred{V}{t}, \textbf{u}_t$
% \begin{algorithmic}[1]
% % \State Align end edges with $\textbf{u}_t$ \Comment{assumption.\ref{assum:grasp condition}}
% \State $\bm{\theta}^*_t(\textbf{X}_t) = \argmin_{\bm{\theta}_t} P(\textbf{X}_t, \bm{\theta}_t,\bm{\alpha})$ \Comment{\secref{sec:Differentiable DER}}
% % \State  $\textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\partial P(\textbf{X}_t, \bm{\theta}_t(\textbf{X}_t),\bm{\alpha}}{\partial  \textbf{X}_{t}}$
% % \Comment{\eqref{eq:Integration}} 
% \State $\hat{\textbf{V}}_{t+1} = \hat{\textbf{V}}_t-\Delta_tM^{-1}\frac{\partial P(\textbf{X}_t, \bm{\theta}^*_t(\textbf{X}_t),\bm{\alpha})}{\partial \textbf{X}_{t}}$ \Comment{\eqref{eq:Semi-Euler2}}   
% \State $\hat{\textbf{X}}_{t+1} = \hat{\textbf{X}}_t + \Delta_t\hat{\textbf{V}}_{t+1} + \text{DNN}$ \Comment{\secref{sec:integration_NN}}
% \State Inextensibility Enforcement on $\hat{\textbf{X}}_{t+1}$ 
% \Comment{\secref{sec:inextensiblity methodology}}
% \State $\hat{\textbf{V}}_{t+1} = (\hat{\textbf{X}}_{t+1} - \hat{\textbf{X}}_t)\Delta_t$ \Comment{Velocity Update}
% \end{algorithmic}
% \Return $\pred{X}{t+1}, \pred{V}{t+1}$
% \end{algorithm}
%     \end{minipage}
%   \end{wrapfigure}

% \begin{wrapfigure}{R}{0.44\textwidth}
% \vspace*{-0.65cm}
%     \begin{minipage}{0.44\textwidth}
% \begin{algorithm}[H]
% \caption{Enforcing Inextensibility with Momentum Preserving PBD} 
% \label{alg:inextensibility of PBD}
% \begin{algorithmic}[1]
% \Require $\pred{X}{t+1}$ and $\epsilon > 0$
% \While {any $\text{C}(\hat{\textbf{x}}^i_{t+1}, \hat{\textbf{x}}^{i+1}_{t+1}) > \epsilon$ }
%     \For{$i = 2$ \textbf{to} $n - 1$}
%         \State $\hat{\textbf{x}}_{t+1}^i = \hat{\textbf{x}}_{t+1}^i + \beta^{i}\Delta \hat{\textbf{x}}_{t+1}^i$ \Comment{\eqref{eq:inext1}}
%         % \State $\hat{\textbf{x}}_{t+1}^\text{i+1} = \hat{\textbf{x}}_{t+1}^\text{i+1} + \beta^{i+1}\Delta \hat{\textbf{x}}_{t+1}^\text{i+1}$ \Comment{\eqref{eq:inext1}}   
%     \EndFor
% \EndWhile
% % \Until{\textbf{all} $||\hat{\textbf{x}}_{t+1}^i - \hat{\textbf{x}}_{t+1}^\text{i+1}|| - ||\overline{\textbf{e}}_i||_2 < threshold$}
% \State \Return: $\hat{\textbf{X}}_{t+1}$ \Comment{Updated Vertices}
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
%   \end{wrapfigure}

% \begin{table}[t]
% \centering
% \caption{A summary of the material properties of each of the wires that were observed/manipulated during the real-world experiment.}
% \label{mat_prop}
% \begin{tabular}{|c||c|c|c|c|}
% \hline
% Name & Length [m] & Weight [g] & Stiffness & \makecell{ \# Mocap \\ Markers}\\ \hline \hline
% DLO 1 & 1.152 & 34.5 & 3 & 13\\ \hline 
% DLO 2 & 0.996 & 65.2 & 4 & 12\\ \hline 
% DLO 3 & 0.998 & 96.8  & 5 & 12 \\ \hline
% DLO 4& 0.973 & 22.0 & 1 & 12\\ \hline 
% DLO 5 & 0.988 & 19.2 & 2 & 12 \\ \hline 
% \end{tabular}
% \end{table}
% \subsection{\Review{}{Motion Planning and Control for DLO Manipulation}{}}



% However, based on experiment and natural deficiency from large-time step discretization, we find that this method cannot capture high dynamic performance. 
% We enhance the integration approach by incorporating predictive compensation. 
% This enhancement is rooted in the concept of residual learning and is achieved through the adaptation of a graph neural network. 
% Further details will be discussed in \secref{sec:integration_NN}.
% ; however, note that our goal is to eventually perform differentiable simulation to allow for auto-tuning certain model parameters which is described in more detail in \secref{sec:Differentiable DER}.

% \subsection{Long Time Horizon Prediction for DLO}

% Following assumptions are made to setup a prediction framework.
% \begin{assum}
%     first two states $\timeind{X}{1}, \timeind{X}{2}$ are fully observable. 
% \end{assum}
% Satisfying this assumption is essential for the initialization of iterative prediction. However, when perception is heavily occluded at the initial state, meeting above assumption can be challenging. Details will be discussed in \secref{section: Estimation}
% \begin{assum}
% End edges of DLO are coupled with grippers such that $\textbf{u}_\text{t}=\{\timevertind{x}{1}{t+1}, \timevertind{x}{2}{t+1}, \timevertind{x}{n-1}{t+1}, \timevertind{x}{n}{t+1}\}$. $\textbf{u}_\text{t}$ can be approximated through inverse kinematics or other perception system.
% \end{assum}
% Above assumption commonly made and well-studied in DLO manipulation among literature\cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}. It provides accessibility and controllability to DLO edges.

%  \Ram{use an assumption environment like in the file I shared with you....} 
% \Ram{what does this mean?}. With above assumptions, denote $F$ as a general modeling function, long-time horizon inference is propagated through iterative prediction as shown in the \textbf{Algorithm} \ref{alg:long time horizon}. Note ground truth is not accessible during the iteration, and all predicted intermediate and final states of the DLO will be used for evaluation. 
% \begin{algorithm}[t]
% \caption{Long Time Horizon Prediction } 
% \label{alg:long time horizon}
% \textbf{Require:} $\textbf{X}_{1:\text{T}}, \textbf{U}_{2:\text{T-1}}$ \Comment{True States and Inputs}\\
% \textbf{Initialization} at t = 2: 
% \begin{algorithmic}[1]
% \State $\textbf{V}_2 = (\textbf{X}_2 - \textbf{X}_1)/\Delta \text{t}$ \Comment{Initial Velocity Estimation } 
% \State $\pred{X}{3} = F(\textbf{u}_2, \textbf{X}_2, \textbf{V}_2)$   \Comment{First Update}
% \State $\pred{V}{3} = (\pred{X}{3} - \textbf{X}_2)/\Delta \text{t}$ \Comment{Velocity Update}
% \State {Iterative Update: $\text{T} \gg \Delta \text{t}$ \Ram{not sure why you need this condition...I think you are just running a for loop? Also isn't this just a single algorithm, why does the line number change halfway thru? Is this supposed to be two algorithms? Then call them two algorithms?}} \Yizhou{I was trying to show it is long time horizon but I can delete this line.}
% \For{$\text{t} \gets 3 \textrm{ to } \text{T}-1$} 
%      \State $\pred{X}{t+1} = F(\textbf{u}_\text{t}, \pred{X}{t}, \pred{V}{t})$
%      \State $\pred{V}{t+1} = (\pred{X}{t+1} - \pred{X}{t})/\Delta t$
% \EndFor
% \State \Return $\pred{X}{3:T}, \, |\pred{X}{3:T} - \timeind{X}{3:T}|$ \Comment{Prediction and Loss}
% \end{algorithmic}
% \end{algorithm}


% \subsection{Integration for DLO Simulation}
% \label{sec:integration}
% Notice that $\theta^*_\text{t}$ is a function of $\timeind{X}{t}$. For conciseness, based on \Eqref{eq:energy}, we note equation of motion as follows: 
% \begin{equation}
%        \textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\delta \text{E}(\Gamma^\text{M}(\timeind{X}{t}))}{\delta \textbf{X}_{t}}
%        \label{eq:Integration}
% \end{equation}
% As DER is not an analytical modeling frame. Solving  \Eqref{eq:Integration} requires numerical integration. DER\cite{originalDER} choose the method to be Semi-Euler method\cite{implicit-euler}, which has the same computational cost while having better tracking performance compared to Euler's method, as shown in the following, 
% \begin{equation}
%         \hat{\textbf{V}}_{t+1} = \textbf{V}_\text{t} -\Delta \text{t}m^{-1}\frac{\delta \text{E}(\Gamma^\text{M}(\textbf{X}_{t}))}{\delta \textbf{X}_{t}}, \, \,  \hat{\textbf{X}}_{\text{t}+1} = \textbf{X}_\text{t} + \Delta \text{t} \hat{\textbf{V}}_{t+1}
%        \label{eq:Semi-Euler}
% \end{equation}
% However, based on experiment and natural deficiency from large-time step discretization, we find that this method cannot capture high dynamic performance. We enhance the integration approach by incorporating predictive compensation. This enhancement is rooted in the concept of residual learning and is achieved through the adaptation of a graph neural network. Further details will be discussed in \secref{sec:integration_NN}.

% \subsection{Long Time Horizon Prediction for DLO}
% Following assumptions are made to setup a prediction framework.
% \begin{assum}
%     first two states $\timeind{X}{1}, \timeind{X}{2}$ are fully observable. 
% \end{assum}
% Satisfying this assumption is essential for the initialization of iterative prediction. However, when perception is heavily occluded at the initial state, meeting above assumption can be challenging. Details will be discussed in \secref{section: Estimation}
% \begin{assum}
% End edges of DLO are coupled with grippers such that $\textbf{u}_\text{t}=\{\timevertind{x}{1}{t+1}, \timevertind{x}{2}{t+1}, \timevertind{x}{n-1}{t+1}, \timevertind{x}{n}{t+1}\}$. $\textbf{u}_\text{t}$ can be approximated through inverse kinematics or other perception system.
% \end{assum}
% Above assumption commonly made and well-studied in DLO manipulation among literature\cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}. It provides accessibility and controllability to DLO edges.

%  \Ram{use an assumption environment like in the file I shared with you....} 
% \Ram{what does this mean?}. With above assumptions, denote $F$ as a general modeling function, long-time horizon inference is propagated through iterative prediction as shown in the \textbf{Algorithm} \ref{alg:long time horizon}. Note ground truth is not accessible during the iteration, and all predicted intermediate and final states of the DLO will be used for evaluation. 
% \begin{algorithm}
% \caption{Long Time Horizon Prediction } 
% \label{alg:long time horizon}
% \textbf{Require:} $\textbf{X}_{1:\text{T}}, \textbf{U}_{2:\text{T-1}}$ \Comment{True States and Inputs}\\
% \textbf{Initialization} at t = 2: 
% \begin{algorithmic}[1]
% \State $\textbf{V}_2 = (\textbf{X}_2 - \textbf{X}_1)/\Delta \text{t}$ \Comment{Initial Velocity Estimation } 
% \State $\pred{X}{3} = F(\textbf{u}_2, \textbf{X}_2, \textbf{V}_2)$   \Comment{First Update}
% \State $\pred{V}{3} = (\pred{X}{3} - \textbf{X}_2)/\Delta \text{t}$ \Comment{Velocity Update}
% \State {Iterative Update: $\text{T} \gg \Delta \text{t}$ \Ram{not sure why you need this condition...I think you are just running a for loop? Also isn't this just a single algorithm, why does the line number change halfway thru? Is this supposed to be two algorithms? Then call them two algorithms?}} \Yizhou{I was trying to show it is long time horizon but I can delete this line.}
% \For{$\text{t} \gets 3 \textrm{ to } \text{T}-1$} 
%      \State $\pred{X}{t+1} = F(\textbf{u}_\text{t}, \pred{X}{t}, \pred{V}{t})$
%      \State $\pred{V}{t+1} = (\pred{X}{t+1} - \pred{X}{t})/\Delta t$
% \EndFor
% \State \Return $\pred{X}{3:T}, \, |\pred{X}{3:T} - \timeind{X}{3:T}|$ \Comment{Prediction and Loss}
% \end{algorithmic}
% \end{algorithm}


% To formulate reduced coordinate modeling, $\theta^\text{i}$ is introduced to measures the rotation about $\vertind{t}{i}$ from Bishop frame $\Gamma^\text{i}_\text{B}: {\{\textbf{t}^\text{i}, \textbf{v}_1^\text{i}, \textbf{v}_2^\text{i}\}}$ relative to material frame material frame $\Gamma^\text{i}_\text{M}:\{\boldsymbol{\textbf{t}}^\text{i}, \textbf{m}_1^\text{i}, \textbf{m}_2^\text{i}\}$ with following equation.
% \begin{equation}
%     \textbf{m}_1^\text{i}=\text{cos}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{sin}\theta^\text{i}\cdot \textbf{v}_2^\text{i}, \textbf{m}_2^\text{i}=-\text{sin}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{cos}\theta^\text{i}\cdot \textbf{v}_2^\text{i}
% \end{equation}
% Bishop frame is referred as twist-free frame according to following lemma:
% \begin{lem}
%     Let $E_\text{twist}(\Gamma^\text{i}(\theta^\text{i}))$ denote twisting energy of $\Gamma^\text{i}$. $\forall \theta^\text{i} \neq 0, E_\text{twist}(\Gamma^\text{i}_\text{M}(\theta^\text{i}))\geq E_\text{twist}(\Gamma^\text{i}_\text{M}(\theta^\text{i}=0)=\Gamma^\text{i}_\text{B})$
% \end{lem}
% Such property is critical as it allows the material frame to use Bishop frame as a reference frame (energy-minimized frame) to capture twisting efficiently. Importantly, bending energy of  material frame has following property.
% \begin{lem}
%     Let $E_\text{bend}(\symbind{\Gamma}{i}(\vertind{e}{i-1}, \vertind{e}{i}, \theta^\text{i})$ denote bending energy of $\symbind{\Gamma}{i}$. $\forall \theta^\text{i} \neq 0, E_\text{bend}(\Gamma^\text{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i},0))\geq E_\text{bend}(\symbind{\Gamma}{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i},\theta^\text{i}))$
% \end{lem}
% Lemma 1 and Lemma 2 allow $\theta^\text{i}$ to distribute twisting and bending energy within a bounded material frame energy. The weight of each is based on quasistatic treatment with the following assumption.
% \begin{assum}
%     The material frame always reaches an equilibrium state before simulating the next step, as $E_\text{twist}(\symbind{\Gamma}{i}_\text{M}(\theta^\text{i})) + E_\text{bend}(\symbind{\Gamma}{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i}, \theta^\text{i}))$ is bounded, $(\symbind{\theta}{i})^*$ can always be solved with following:
%     \begin{equation}
%         (\symbind{\theta}{i})^* = \underset{\theta^i}{\arg\min}(E_\text{twist}(\symbind{\Gamma}{i}_\text{M}(\theta^\text{i})) + E_\text{bend}(\symbind{\Gamma}{i}_\text{M}(\vertind{e}{i-1}, \vertind{e}{i},\theta^\text{i})))
%         \label{eq:opt_theta}
%     \end{equation}
% \end{assum}
% Final energy is expressed as following:
% \begin{equation}
%     \text{E}(\Gamma^\text{M}(\theta^*), \textbf{E}) = \sum^{n-1}_{i=2}\text{E}_{\text{twist}}(\Gamma_\text{M}^\text{i}((\symbind{\theta}{i})^*)) + \text{E}_{\text{bend}}(\Gamma_\text{M}^{i}(\vertind{e}{i-1}, \vertind{e}{i}, (\symbind{\theta}{i})^*)) 
%     \label{eq:energy}
% \end{equation}
% Such energy formulation in reduced coordinates facilitates computation efficiency while managing to perform bending and twisting. Despite its success, notice we want to build a differentiable simulation that enables parameter auto-tuning. However, solving of Eq.\ref{eq:opt_theta} poses challenge to obtain gradients, which will be discussed in \secref{sec:Differentiable DER}.


% \subsection{Integration for DLO Simulation}
% \label{sec:integration}
% Notice that $\theta^*_\text{t}$ is a function of $\timeind{X}{t}$. For conciseness, based on \Eqref{eq:energy}, we note equation of motion as follows: 
% \begin{equation}
%        \textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\delta \text{E}(\Gamma^\text{M}(\timeind{X}{t}))}{\delta \textbf{X}_{t}}
%        \label{eq:Integration}
% \end{equation}
% As DER is not an analytical modeling frame. Solving  \Eqref{eq:Integration} requires numerical integration. DER\cite{originalDER} choose the method to be Semi-Euler method\cite{implicit-euler}, which has the same computational cost while having better tracking performance compared to Euler's method, as shown in the following, 
% \begin{equation}
%         \hat{\textbf{V}}_{t+1} = \textbf{V}_\text{t} -\Delta \text{t}m^{-1}\frac{\delta \text{E}(\Gamma^\text{M}(\textbf{X}_{t}))}{\delta \textbf{X}_{t}}, \, \,  \hat{\textbf{X}}_{\text{t}+1} = \textbf{X}_\text{t} + \Delta \text{t} \hat{\textbf{V}}_{t+1}
%        \label{eq:Semi-Euler}
% \end{equation}
% However, based on experiment and natural deficiency from large-time step discretization, we find that this method cannot capture high dynamic performance. We enhance the integration approach by incorporating predictive compensation. This enhancement is rooted in the concept of residual learning and is achieved through the adaptation of a graph neural network. Further details will be discussed in \secref{sec:integration_NN}.

% \subsection{Long Time Horizon Prediction for DLO}
% Following assumptions are made to setup a prediction framework.
% \begin{assum}
%     first two states $\timeind{X}{1}, \timeind{X}{2}$ are fully observable. 
% \end{assum}
% Satisfying this assumption is essential for the initialization of iterative prediction. However, when perception is heavily occluded at the initial state, meeting above assumption can be challenging. Details will be discussed in \secref{section: Estimation}
% \begin{assum}
% End edges of DLO are coupled with grippers such that $\textbf{u}_\text{t}=\{\timevertind{x}{1}{t+1}, \timevertind{x}{2}{t+1}, \timevertind{x}{n-1}{t+1}, \timevertind{x}{n}{t+1}\}$. $\textbf{u}_\text{t}$ can be approximated through inverse kinematics or other perception system.
% \end{assum}
% Above assumption commonly made and well-studied in DLO manipulation among literature\cite{IRP, diminishingridgidity, directionalrigidity, inlstm, gelsim}. It provides accessibility and controllability to DLO edges.

%  \Ram{use an assumption environment like in the file I shared with you....} 
% \Ram{what does this mean?}. With above assumptions, denote $F$ as a general modeling function, long-time horizon inference is propagated through iterative prediction as shown in the \textbf{Algorithm} \ref{alg:long time horizon}. Note ground truth is not accessible during the iteration, and all predicted intermediate and final states of the DLO will be used for evaluation. 
% \begin{algorithm}
% \caption{Long Time Horizon Prediction } 
% \label{alg:long time horizon}
% \textbf{Require:} $\textbf{X}_{1:\text{T}}, \textbf{U}_{2:\text{T-1}}$ \Comment{True States and Inputs}\\
% \textbf{Initialization} at t = 2: 
% \begin{algorithmic}[1]
% \State $\textbf{V}_2 = (\textbf{X}_2 - \textbf{X}_1)/\Delta \text{t}$ \Comment{Initial Velocity Estimation } 
% \State $\pred{X}{3} = F(\textbf{u}_2, \textbf{X}_2, \textbf{V}_2)$   \Comment{First Update}
% \State $\pred{V}{3} = (\pred{X}{3} - \textbf{X}_2)/\Delta \text{t}$ \Comment{Velocity Update}
% \State {Iterative Update: $\text{T} \gg \Delta \text{t}$ \Ram{not sure why you need this condition...I think you are just running a for loop? Also isn't this just a single algorithm, why does the line number change halfway thru? Is this supposed to be two algorithms? Then call them two algorithms?}} \Yizhou{I was trying to show it is long time horizon but I can delete this line.}
% \For{$\text{t} \gets 3 \textrm{ to } \text{T}-1$} 
%      \State $\pred{X}{t+1} = F(\textbf{u}_\text{t}, \pred{X}{t}, \pred{V}{t})$
%      \State $\pred{V}{t+1} = (\pred{X}{t+1} - \pred{X}{t})/\Delta t$
% \EndFor
% \State \Return $\pred{X}{3:T}, \, |\pred{X}{3:T} - \timeind{X}{3:T}|$ \Comment{Prediction and Loss}
% \end{algorithmic}
% \end{algorithm}



% The bishop frame is defined as following:
% \begin{defn}
%     \label{def: Bishop}
%      Denote $\bm{v^\text{i+1}} = R_{\text{q}^\text{i}}(\bm{v^\text{i}}), \, \text{q}^\text{i}=(\text{q}_0^\text{i}, \textbf{q}^\text{i})$ as quaternion rotation that rotates $\bm{v^\text{i}}$ around axial vector $\textbf{q}^\text{i}$ with magnitude $\text{q}_0^\text{i}$. Let $\phi^\text{i}$ denote the turning angle between $\vertind{e}{i}$ and $\vertind{e}{i+1}$. Given 
% \begin{equation}
% \textbf{t}^{\text{i}+1} =R_{\text{q}^\text{i}}(\textbf{t}^\text{i}),\, \textbf{n}_1^{\text{i}+1} \label{eq:parallel transfort1} =R_{\text{q}^\text{i}}(\textbf{n}_1^\text{i})
% \end{equation}  
% \begin{equation}
% \text{q}_0^\text{i} = \text{cos}(\phi^\text{i}/2), \, \textbf{q}^\text{i} = \text{sin}(\phi^\text{i}/2)(\textbf{t}^\text{i} \times \textbf{t}^{\text{i}+1})
% \label{eq:parallel transfort2}    
% \end{equation}
% A frame that is transported with above equations is Bishop frame $\Gamma^\text{i}_\text{B}: {\{\textbf{t}, \textbf{v}_1, \textbf{v}_2\}}$.
% % \end{defn}
% \begin{defn}
%     \label{def: material frame}
%     Let a rotation angle $\vertind{$\theta$}{i}$ that represents rotation from Bishop frame to material frame $\Gamma^\text{i}_\text{M}:{\{\boldsymbol{\textbf{t}}^\text{i}, \textbf{m}_1^\text{i}, \textbf{m}_2^\text{i}}\}$ about $\vertind{t}{i}$ with the following equation.
% \begin{equation}
%     \textbf{m}_1^\text{i}=\text{cos}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{sin}\theta^\text{i}\cdot \textbf{v}_2^\text{i}, \textbf{m}_2^\text{i}=-\text{sin}\theta^\text{i}\cdot \textbf{v}_1^\text{i} + \text{cos}\theta^\text{i}\cdot \textbf{v}_2^\text{i}
% \end{equation}



\begin{wrapfigure}{R}{0.6\textwidth}
      \vspace*{-0.65cm}
    \begin{minipage}{0.6\textwidth}
      \begin{algorithm}[H]
\caption{One Step Prediction} 
\label{alg:long time horizon}
\textbf{Inputs}: $\pred{X}{t}, \pred{V}{t}, \textbf{u}_t$
\begin{algorithmic}[1]
% \State Align end edges with $\textbf{u}_t$ \Comment{assumption.\ref{assum:grasp condition}}
\State $\bm{\theta}^*_t(\textbf{X}_t) = \argmin_{\bm{\theta}_t} P(\textbf{X}_t, \bm{\theta}_t,\bm{\alpha})$ \Comment{\secref{sec:Differentiable DER}}
% \State  $\textit{\textbf{M}}\ddot{\textbf{X}}_{t} = -\frac{\partial P(\textbf{X}_t, \bm{\theta}_t(\textbf{X}_t),\bm{\alpha}}{\partial  \textbf{X}_{t}}$
% \Comment{\eqref{eq:Integration}} 
\State $\hat{\textbf{V}}_{t+1} = \hat{\textbf{V}}_t-\Delta_tM^{-1}\frac{\partial P(\textbf{X}_t, \bm{\theta}^*_t(\textbf{X}_t),\bm{\alpha})}{\partial \textbf{X}_{t}}$ \Comment{\eqref{eq:Semi-Euler2}}   
\State $\hat{\textbf{X}}_{t+1} = \hat{\textbf{X}}_t + \Delta_t\hat{\textbf{V}}_{t+1} + \text{DNN}$ \Comment{\secref{sec:integration_NN}}
\State Inextensibility Enforcement on $\hat{\textbf{X}}_{t+1}$ 
\Comment{\secref{sec:inextensiblity methodology}}
\State $\hat{\textbf{V}}_{t+1} = (\hat{\textbf{X}}_{t+1} - \hat{\textbf{X}}_t)\Delta_t$ \Comment{Velocity Update}
\end{algorithmic}
\Return $\pred{X}{t+1}, \pred{V}{t+1}$
\end{algorithm}
    \end{minipage}
  \end{wrapfigure}

%   \begin{figure}[t]
%     \centering
%     % First row
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp_res_1.pdf}
%         \caption{DLO 1, robot-human manipulation}
%         \label{fig:rh_thin}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp_res_2.pdf}
%         \caption{DLO 1, dual-robot manipulation}
%         \label{fig:rr_thin}
%     \end{subfigure}
%     \vspace{0.2cm}

%     % Second row
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp_res_3.pdf}
%         \caption{DLO 2, robot-human manipulation}
%         \label{fig:rh_thick}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp_res_4.pdf}
%         \caption{DLO 2, dual-robot manipulation}
%         \label{fig:rr_thick}
%     \end{subfigure}
%     \vspace{0.2cm}

%     % Third row
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp_res_5.pdf}
%         \caption{DLO 3, robot-human manipulation}
%         \label{fig:rh_aniso}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/exp_res_6.pdf}
%         \caption{DLO 3, dual-robot manipulation}
%         \label{fig:rr_aniso}
%     \end{subfigure}
%     \vspace{0.2cm}
%     \vspace{-0.2cm}

%     \caption{Visualization of the performance of DEFORM and Bi-LSTM in predicting trajectories for DLOs 1 \Revise{, 2, and 3}{}. The ground truth vertices of the DLOs are marked with red hollow circles. The predicted vertices are marked with orange solid circles for DEFORM and blue solid circles for the Bi-LSTM model, respectively.}
%     \label{fig:grid}
% \end{figure}
